Estimating Social Influence from Observational Data

We consider the problem of estimating social influence, the effect that a person's behavior has on the future behavior of their peers. The key challenge is that shared behavior between friends could be equally explained by influence or by two other confounding factors: 1) latent traits that caused people to both become friends and engage in the behavior, and 2) latent preferences for the behavior. This paper addresses the challenges of estimating social influence with three contributions. First, we formalize social influence as a causal effect, one which requires inferences about hypothetical interventions. Second, we develop Poisson Influence Factorization (PIF), a method for estimating social influence from observational data. PIF fits probabilistic factor models to networks and behavior data to infer variables that serve as substitutes for the confounding latent traits. Third, we develop assumptions under which PIF recovers estimates of social influence. We empirically study PIF with semi-synthetic and real data from Last.fm, and conduct a sensitivity analysis. We find that PIF estimates social influence most accurately compared to related methods and remains robust under some violations of its assumptions.

==> intro.tex <==
\section{Introduction}
\label{sec:introduction}

This paper is about analyzing social network data to estimate
social influence, the effect that its members have on each other. 
How does the past
behavior of a person in a network influence the current behavior of
their peers?
Researchers across many fields have studied questions that involve social influence.
For example, \citet{bond2012voter} study whether Facebook users influence their friends to vote in elections;
\citet{christakis2007obesity} ask whether a person's obesity status affects those of their family and friends;
\citet{bakshy2012social} study whether social influence increases the effectiveness of an ad campaign.

We develop Poisson Influence Factorization (PIF), a new
method for estimating social influence.
PIF analyzes a social network, the past behavior of its
members, and the current behavior of its members to
estimate each person's social influence.
To measure a behavior of interest, such as product consumption, we use multivariate data, such as the purchases of many items.
PIF can be applied to study social influence in many settings including Facebook users sharing news articles, Twitter users using hashtags, or e-commerce site users purchasing products.
To explain ideas, we will use the example of people purchasing items throughout the paper.

This paper makes three main contributions.  The first is to frame the
problem of estimating social influence as a causal inference, 
a question about a hypothetical world created by intervening upon variables in a system.
Informally, to define the social influence of a person on their peer, we ask:
if we could have ``made'' the person buy an item yesterday, would their peer purchase the item today?
Intuitively, for a person who has social influence, if we hypothetically intervene to make them buy an item yesterday, we expect that their peer is more likely to buy the item today.

The second contribution is to introduce the assumptions
from which we can estimate social influence with observational data.
In an observed dataset of a network and the purchases of its members,
we cannot intervene on people yesterday and observe the outcomes of their peers.
Instead, several factors, called confounders, affect what people purchase yesterday and what their
peers purchase today.
Confounders create a correlation between people's behavior that is not driven by social influence.
We articulate the assumptions needed to distinguish the causal effect of social influence
from the effects of confounders.

The third contribution is the PIF algorithm
for estimating social influence from observed networks.
The challenge with estimating social influence is that the confounders
are usually unobserved.
However, the confounders drive the observed purchases and connections in the network.
We operationalize this insight by fitting well-studied statistical models of networks such as community models \citep{ball2011efficient,gopalan2013efficient,contisciani2020} or stochastic block models \citep{holland1983stochastic,peixoto2019bayesian,airoldi2008mixed,karrer2011stochastic}. We will show how these models produce variables that contain some of the same information as the confounders.
PIF uses these variables to reduce the bias due to confounders when estimating social influence.

To understand the challenges with estimating social influence, consider the following example:
\begin{example}
	\label[example]{eg:sports_drink}
	We observe that yesterday, \personi{} bought a sports drink and today, her friend \personj{} bought
	the same sports drink. Did \personi{} influence \personj{} to buy the
	drink or would \personj{} have bought it anyway?
\end{example}
The problem is that the shared purchasing behavior between \personi{} and \personj{} might be explained in different ways.
\personi{} and \personj{} became friends because of their shared interest in sports and this interest caused them each to buy the drink. 
(The idea that people with shared traits are more likely to connect is known as homophily.)
Alternatively, \personi{} and \personj{} might both happen to like sports drinks, even though they became friends because they live in the same building.
It is their preference for sports drinks that drives their purchases, irrespective of the reasons they became friends.
Finally, \personi{} might have caused \personj{} to buy the drink because of her social influence.
The shared purchasing behavior might be evidence for social influence, but it might arise from the two other reasons.
Thus, the factors that cause people to form a connection and purchase items are confounders of social influence.

When all confounders are observed, there are well-known techniques that yield valid causal inferences \cite{Pearl:2009a,rosenbaum1983central,rubin2005causal}. \citet{ogburn2017social,sharma2016distinguishing,eckles2020bias,aral2009distinguishing} adapt these techniques for the social influence setting when the confounders are assumed to be observed.
However, \citet{shalizi2011homophily} caution that is usually difficult to observe all confounders; unobserved factors that drive connections and purchases can still bias our estimates of social influence. PIF works in the context of this problem.

%However, from observed social networks and data about yesterday and today's purchases, where unobserved factors drive preference and homophily, estimating social influence is impossible without other assumptions.

%To develop assumptions in service of estimating social influence, 
%PIF uses the fact that unobserved confounders drive the observed connections and purchases.

The main idea behind PIF is that the unobserved confounders, though
not explicitly coded in the data, drive the observed connections between people and their purchases.
PIF makes assumptions about the structure of these relationships, and then uses probabilistic models of networks and purchases to estimate 
variables that contain some of the same
information as the unobserved confounders.
We can then use these estimated variables in 
existing causal inference techniques to 
estimate social influence.

In using latent variable models to estimate variables that can be used in causal inference,
PIF adapts and extends ideas from
\citet{Wang:Blei:2019,Shalizi:McFowland:2016}.
Building on their work, we show that models of both networks and purchases are needed to adjust
for the bias due to confounders.
\citet{chaney2015probabilistic} extend latent variable models to model purchases based on both social networks and unobserved preferences, but they do not consider causal inference of social influence.
In different causal inference settings, \citet{guo2020learning,veitch2019using} have also used
inferred properties of social networks as estimates of confounders.

We study PIF empirically with semi-synthetic
simulations, using a novel procedure that uses real social networks to
synthesize different purchasing scenarios under varying amounts of
confounding.  We find that PIF is more accurate at recovering
influence than related methods.  
Finally, we apply PIF to real data from the song-sharing platform
Last.fm to perform an exploratory study.
We find evidence of correlated song-listening behavior between friends,
but the results from PIF suggest that most of it is attributed to shared preferences
and influence plays a small role.
Code and data will be publicly available.

At the intersection of causality and networks, there are two other lines of work that are distinct to this paper.
First, there is work on the bias introduced by social networks when estimating causal effects \citep{ogburn2017social,sherman2018identification,sherman2020general}.
In this line of work, social influence is an obstacle to valid inference, inducing dependence across people in the network.
In this paper, however, social influence is itself the target of causal inference.
Second, there is work on estimating social influence from time series data \citep{soni2019cascades,anagnostopoulos2008influence,laFond2010randomization} or randomized experiments in social networks \citep{aral2012identifying,aral2013engineering,taylor2013selection,toulis2013estimation}.
In contrast, we focus on the observational setting in this paper.
%However, in observational data, estimating social influence in the presence of unobserved confounders is not possible without further assumptions.

==> preamble_math_short.tex <==
%\DeclareRobustCommand{\mb}[1]{\mathbold{#1}}
\DeclareRobustCommand{\mb}[1]{\boldsymbol{#1}}

\newcommand{\argmax}{arg\,max}
\newcommand{\argmin}{arg\,min}

%\DeclareMathOperator*{\diag}{diag}

\newcommand{\cyan}[1]{{\color{cyan}{#1}\normalcolor}}
\newcommand{\yellow}[1]{{\color{yellow}{#1}\normalcolor}}
%\newcommand{\red}[1]{{\color{red}{#1}\normalcolor}}
%\newcommand{\magenta}[1]{{\color{magenta}{#1}\normalcolor}}
%\newcommand{\green}[1]{{\color{green}{#1}\normalcolor}}
%\newcommand{\blue}[1]{{\color{blue}{#1}\normalcolor}}

\newcommand{\vv} {{\bm v}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}} 
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}

\newcommand{\e}{\mathrm{e}}
\renewcommand{\L}{\mathcal{L}}
\renewcommand{\vec}[1]{#1}

\newcommand{\mbeq}{\stackrel{!}{=}} % "mbeq": must be equal

\newcommand{\Gam}{\textrm{Gam}}
\newcommand{\multi}{\textrm{Mult}}
\newcommand{\Dir}{\textrm{Dir}}
\newcommand{\discrete}{\textrm{Discrete}}
\newcommand{\Bern}{\textrm{Bern}}
\newcommand{\DP}{\textrm{DP}}
\newcommand{\GP}{\textrm{GP}}
\newcommand{\Bet}{\textrm{Beta}}
\newcommand{\const}{\mathrm{const}}
\newcommand{\pois}{\textrm{Pois}}
\newcommand{\gauss}{\textrm{Gauss}}


\newcommand*{\tens}[1]{\underline{\mathbf{#1}}}

\newcommand{\bs}{\mathbf{s}}

\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\balpha}{\mb{\alpha}}
\newcommand{\bbeta}{\mb{\beta}}
\newcommand{\bmu}{\mb{\mu}}
\newcommand{\bsigma}{\mb{\sigma}}
\newcommand{\btheta}{\mb{\theta}}
\newcommand{\blambda}{\mb{\lambda}}
\newcommand{\bgamma}{\mb{\gamma}}
\newcommand{\bphi}{\mb{\phi}}
\newcommand{\btau}{\mb{\tau}}
\newcommand{\bbbeta}{\mb{\eta}}
\newcommand{\bpi}{\mb{\pi}}
\newcommand{\bepsilon}{\mb{\epsilon}}
\newcommand{\bzeta}{\mb{\zeta}}
\newcommand{\bvarphi}{\mb{\varphi}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bnu}{\mathbf{\nu}}
\newcommand{\bkappa}{\mathbf{\kappa}}
\newcommand{\bomega}{\mathbf{\omega}}
\newcommand{\ELBO}{\textsc{elbo}}
\newcommand{\cQ}{\mathcal{Q}}

\newcommand{\cD}{{\cal D}} 
\newcommand{\cL}{{\cal L}} 
\newcommand{\cM}{{\cal M}} 
\newcommand{\cN}{{\cal N}} 
\newcommand{\cO}{{\cal O}} 
\newcommand{\cU}{{\cal U}} 
\newcommand{\cW}{{\cal W}} 
\newcommand{\cZ}{{\cal Z}} 
\newcommand{\loglik}{\mathcal{L}}
\newcommand{\grad}{{\nabla}} 



\let\vaccent=\v % rename builtin command \v{} to \vaccent{}
\renewcommand{\v}[1]{\mathbf{#1}} % for vectors
\renewcommand{\bf}[1]{\textbf{#1}} % for bold words

\newcommand{\ra}{\rightarrow}
\newcommand{\f}[2]{\frac{#1}{#2}}
\newcommand{\avg}[1]{\left\langle #1 \right\rangle} % for average
\let\setunion=\ccup
\newcommand{\ccup}[1]{\left\{#1\right\}}
\let\setunion=\bup
\let\setunion=\rup
\newcommand{\bup}[1]{\left(#1\right)}
\newcommand{\rup}[1]{\left[#1\right]}

\let\oldt=\t
\renewcommand{\t}[1]{\tilde{#1}}
\newcommand{\w}{\omega}
\newcommand{\bb}[1]{\mathbf{#1}}
\newcommand{\s}{\sigma}
\newcommand{\tm}{\times}
\newcommand{\al}{\alpha}
\renewcommand{\b}[1]{\bar{#1}}
\newcommand{\h}[1]{\hat{#1}}

\newcommand{\id}{\mathbb{I}}
%\newcommand{\e}{\mathrm{e}}
\newcommand{\Exp}{\mathbb{E}}
\renewcommand{\mid}{\,|\,}
\newcommand{\eps}{\sigma} 
\newcommand{\ones}{\mathbf{1}}

\renewcommand{\ref}[1]{[\ref{#1}]}


==> preamble_usepackage_short.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our additions of packages: 

% TABLES
\usepackage{tabularx}

\usepackage{amsfonts,amsmath,amssymb}   % clashes with mathdesign
%\usepackage{amsmath,fixmath}
\usepackage{comment}
\usepackage{lineno}
\usepackage{hyperref}
\usepackage[explicit]{titlesec}

% FIGURES
%\usepackage[caption=false]{subfig}
\usepackage{graphicx}
\usepackage[labelfont=bf]{caption}
\usepackage[format=hang]{subcaption}

% ALGORITHMS
\usepackage{algorithm,algorithmic}

%\usepackage{csvsimple}
%\usepackage{filecontents}
%
%	
\hypersetup{
 bookmarks=true, % show bookmarks bar?
 unicode=false, % non-Latin characters in Acrobat�s bookmarks
 pdftoolbar=true, % show Acrobat�s toolbar?
 pdfmenubar=true, % show Acrobat�s menu?
 pdffitwindow=false, % window fit to page when opened
 pdfstartview={FitH}, % fits the width of the page to the window
 pdftitle={}, % title
 pdfauthor={}, % author
 pdfcreator={}, % creator of the document
 pdfproducer={}, % producer of the document
 pdfkeywords={} {} {}, % list of keywords
 pdfnewwindow=true, % links in new window
 colorlinks=true, % false: boxed links; true: colored links
 linkcolor=red, % color of internal links
 citecolor=blue, % color of links to bibliography
 filecolor=magenta, % color of file links
 urlcolor=cyan % color of external links
}
